FiFo: Fishbone Forwarding in Massive IoT Networks

Massive Internet of Things (IoT) networks have a wide range of applications, including but not limited to the rapid delivery of emergency and disaster messages. Although various benchmark algorithms have been developed to date for message delivery in such applications, they pose several practical challenges such as insufficient network coverage and/or highly redundant transmissions to expand the coverage area, resulting in considerable energy consumption for each IoT device. To overcome this problem, we first characterize a new performance metric, forwarding efficiency, which is defined as the ratio of the coverage probability to the average number of transmissions per device, to evaluate the data dissemination performance more appropriately. Then, we propose a novel and effective forwarding method, fishbone forwarding (FiFo), which aims to improve the forwarding efficiency with acceptable computational complexity. Our FiFo method completes two tasks: 1) it clusters devices based on the unweighted pair group method with the arithmetic average; and 2) it creates the main axis and sub axes of each cluster using both the expectation-maximization algorithm for the Gaussian mixture model and principal component analysis. We demonstrate the superiority of FiFo by using a real-world dataset. Through intensive and comprehensive simulations, we show that the proposed FiFo method outperforms benchmark algorithms in terms of the forwarding efficiency.

==> secions_final/references.tex <==
\bibliographystyle{IEEEtran}

\begin{thebibliography}{1}

\bibitem{MassiveIoT01}
F. Guo, F. R. Yu, H. Zhang, X. Li, H. Ji and V. C. M. Leung, ``Enabling massive IoT toward 6G: A comprehensive survey," \emph{IEEE Internet Things J.}, vol. 8, no. 15, pp. 11891-11915, Aug. 2021.

\bibitem{MassiveIoT02}
D. C. Nguyen et al., ``6G Internet of Things: A comprehensive survey," \emph{IEEE Internet Things J.}, Early Access, Aug. 2021.

\bibitem{Oulu}
M. Latva-aho and K. Leppänen (ed.), "Key  drivers and research challenges for 6G ubiquitous wireless intelligence (white paper)". Oulu, Finland \emph{6G Flagship1}, pp. 1-36, Sep. 2019.

\bibitem{Whatis5G}
H. Yu, H. Lee, and H. Jeon, ``What is 5G? Emerging 5G mobile services and network requirements," \emph{MDPI Sustainability}, vol. 9, no. 10, pp. 1-22, Oct. 2017.

\bibitem{D2D1} 
A. Asadi, Q. Wang, and V. Mancuso, ``A survey on device-to-device communication in cellular networks," \emph{IEEE Commun. Surveys Tuts.}, vol.~16, pp.~1801--1819, 2014.

\bibitem{D2D2} 
S. Andreev, A. Pyattaev, K. Johnsson, O. Galinina, and Y. Koucheryavy, ``Cellular traffic offloading onto network-assisted device-to-device connections," \emph{IEEE Commun. Mag.}, vol.~52, pp.~20--31, Apr. 2014.

\bibitem{epidemic} 
A. Vahdat and D. Becker, ``Epidemic routing for partially-connected ad hoc networks," \emph{Duke University}, Jul. 2000.

\bibitem{BIP} 
J. E. Wieselthier, G. D. Nguyen and A. Ephremides, ``On the construction of energy-efficient broadcast and multicast trees in wireless networks," in \emph{Proceedings IEEE INFOCOM 2000. Conference on Computer Communications. Nineteenth Annual Joint Conference of the IEEE Computer and Communications Societies (Cat. No.00CH37064)}, Tel Aviv, Israel,  pp. 585-594, vol. 2, Mar. 2000.

\bibitem{DelegationForwarding}
v. Erramilli, M. Crovella, A. Chaintreau, and C. Diot, ``Delegation forwarding," in \emph{ACM MobiHoc 2008}, Hong Kong SAR, China, pp. 251-260, Jan. 2008.

\bibitem{BroadcastStorm}
Y.-C. Tseng, S.-Y. Ni, Y.-S. Chen, and J.-P. Sheu, ``The broadcast storm problem in a mobile ad hoc network," \emph{Wireless Netw.}, vol. 8, pp. 153--167, Mar. 2002.

\bibitem{BulkDataDissemination}
X. Zheng, J. Wang, W. Dong, Y. He, and Y. Liu, ``Bulk data dissemination in wireless sensor networks: {A}nalysis, implications and improvement," \emph{IEEE Trans. Computers}, vol. 65, no. 5, pp. 1428--1439, May 2016.

\bibitem{CBR}
S. Pal and S. Misra, ``Contact-based routing in DTNs,” in \emph{ACM IMCOM},Bali, Indonesia, no. 3, pp. 1-6, Jan. 2015.

\bibitem{SEBAR}
F. Li, H. Jiang, H. Li, Y. Cheng, and Y. Wang, ``SEBAR: Social-energy-based routing for mobile social delay-tolerant networks," \emph{IEEE Trans. Veh. Technol.}, vol. 66, no. 8, pp. 7195-7206, Aug. 2017.

\bibitem{Coff}
Z. Li, Y. Liu, H. Zhu and L. Sun, ``Coff: Contact-duration-aware cellular traffic offloading over delay tolerant networks," \emph{IEEE Trans. Veh. Technol.}, vol. 64, no. 11, pp. 5257-5268, Nov. 2015.

\bibitem{SeeR}
B. K. Saha, S. Misra and S. Pal, ``SeeR: Simulated annealing-based routing in opportunistic mobile networks," \emph{IEEE Trans. Mobile Comput.}, vol. 16, no. 10, pp. 2876-2888, Oct. 2017.

\bibitem{Weberetal} 
S. P. Weber, X. Yang, J. G. Andrews, G. de
Veciana, ``Transmission capacity of wireless ad hoc networks with
outage constraints," \emph{IEEE Trans. Inf. Theory}, vol. 51, no. 12, pp. 4091-4102, Dec. 2005

\bibitem{Stoyanetal} 
D. Stoyan, W. S. Kendall, J. Mecke,
\emph{Stochastic geometry and its applications.} UK: John Wiley \& Sons,Ltd, 1995.

\bibitem{Shinetal} 
W.-Y. Shin, B. C. Singh, J. Cho, A. M. Everett,
``A new understanding of friendships in space: Complex networks meet
Twitter," \emph{J. Inf. Sci.}, vol. 41, no. 6, pp.751-764, Nov. 2015.

\bibitem{Kwaketal} 
H. Kwak, C. Lee, H. Park, S. Moon, ``What is
Twitter, a social network or a news media?," in \emph{ACM WWW}, Raleigh, North Carolina, USA, pp. 591-600, Apr. 2010,

\bibitem{PCA} 
Ian Jolliffe, ``Principal component analysis," in \emph{International encyclopedia of statistical science}, Berlin, Heidelberg: Springer, 2011, pp.1094--1096.


\bibitem{GMM} 
Douglas Reynolds, ``Gaussian mixture models." \emph{Encyclopedia of biometrics}, Springer, 2015, pp. 827-832.

\bibitem{Mahalanobis} 
R. De Maesschalck, D. Jouan-Rimbaud, and D.L. Massart. ``The Mahalanobis distance." \emph{Chemometrics and intelligent laboratory systems}, vol. 50, no. 1, pp. 1-18, 2000.

\bibitem{UPGMA} 
William H. E. Day and H. Edelsbrunner. ``Efficient algorithms for agglomerative hierarchical clustering methods." \emph{Journal of classification}, vol. 1, no. 1, pp. 7-24, 1984.

\bibitem{EMPCA} 
Sam Roweis, ``EM algorithms for PCA and SPCA." \emph{Advances in neural information processing systems}, Denver, CO, USA, pp. 626-632, 1998.

\bibitem{EMPCA2}
Lindsay I Smith, ``A tutorial on principal components analysis.", University of Otago, New Zealand, OUCS-2002-12, May, 2002.


\bibitem{BIPCOMPLEXITY}
Jeffrey E. Wieselthier, Gam D. Nguyen, and Anthony Ephremides. ``Energy-efficient broadcast and multicast trees in wireless networks," \emph{Mobile networks and applications},vol. 7, no. 6, pp.481-492, 2002.

\bibitem{UPGMAcomplexity}
F. Murtagh, ``Complexities of hierarchic clustering algorithms: State of the art," \emph{Computational Statistics Quarterly}, vol. 1, no. 2, pp. 101-113, 1984.


\bibitem{NPB}
Liu, Wei, Kiyohide Nakauchi, and Yozo Shoji. ``A neighbor-based probabilistic broadcast protocol for data dissemination in mobile IoT networks,`` \emph{IEEE Access}, vol. 6, pp.12260-12268, 2018.


\end{thebibliography}
